A Neural Attention Model for Abstractive Sentence Summarization

Summarization based on text extraction is inherently limited, but generation-style abstractive methods have proven challenging to build. In this work, we propose a fully data-driven approach to abstractive sentence summarization. Our method utilizes a local attention-based model that generates each word of the summary conditioned on the input sentence. While the model is structurally simple, it can easily be trained end-to-end and scales to a large amount of training data. The model shows significant performance gains on the DUC-2004 shared task compared with several strong baselines.

==> lexical.tex <==
\section{Lexical Features}

While a system based on lexical embeddings has several benefits one issue is that it can have trouble handling rare words \cite{}. For MT, one solution to this problem is to utilize an alignment to transfer words directly \cite{}. In Summarization, we can simply reproduce the words from the input directly. We do this by modifying the final soft-max of the model to include ``features'' for each of the original input words.   

\[ p(\yvec_{i+1} | \context, \xvec) \propto \exp(\Vvec \hvec + \Wvec \mathrm{enc}(\context, \xvec) + \alpha \sum_{i} \xvec_i )  \]

In fact we can take this approach a step further and add a small set of additional features,

\[ p(\yvec_{i+1} | \context, \xvec) \propto \exp(\Vvec \hvec + \Wvec \mathrm{enc}(\context, \xvec) + \alpha^\top f(\xvec, \yvec) ).  \]

We include 5 features which indicate,

\begin{itemize}
\item Length of the output.
\item Unigram, bigram, and trigram matches with input
\item Reorderings of the input.
\end{itemize}

During training  

